HiRAE: Hierarchical Representation Autoencoding with Residual Budgets

Pretrained visual representations support image generation, but may not fully preserve the fine-grained details needed for faithful reconstruction. Meanwhile, intermediate encoder layers contain complementary visual details, but learning to fuse them for reconstruction can produce a latent distribution that is difficult to model. Existing fusion methods require empirical tuning of layer selection or staged optimization of fusion and decoding, increasing configuration effort or training complexity. We introduce HiRAE (Hierarchical Representation Autoencoder), which learns a hierarchical fusion framework over the full encoder hierarchy to improve reconstruction fidelity while maintaining compatibility with generative modeling. HiRAE groups encoder layers by depth and learns residual corrections to the deepest representation. Group-wise norm caps bound these corrections relative to the deep anchor, with tighter budgets for shallower groups. Our HiRAE-24 preserves the latent token count and channel dimension. On ImageNet-256, HiRAE-24 reduces reconstruction FID from 0.299 to 0.209 relative to RAEv2 while maintaining competitive guided generation quality. For text-to-image generation, HiRAE-24 improves alignment over RAEv2 on GenEval, DPG-Bench, and GenAI-Bench both before and after supervised fine-tuning. Under the same generator-training and evaluation protocol, post-fine-tuning GenEval increases from 84.86 to 87.70.

==> HiRAE_Arxiv/analysis/tables/edge_reconstruction.tex <==
\begin{tabular}{lrr}
\toprule
Tokenizer & Sobel MSE $\downarrow$ & Laplacian MSE $\downarrow$\\
\midrule
RAEv2 & 1.830 & 43.378\\
HiRAE-7 & 1.167 & 36.124\\
HiRAE-24 & \textbf{0.816} & \textbf{32.645}\\
\bottomrule
\end{tabular}


==> HiRAE_Arxiv/analysis/tables/full_depth_composition.tex <==
\begin{tabular*}{\linewidth}[t]{@{}l@{\extracolsep{\fill}}rrr@{}}
\toprule
Metric & \shortstack{DRoRAE-style\\fusion} & HiRAE-24 & Reduction\\
\midrule
\multicolumn{4}{@{}l}{\textit{20 generator epochs}}\\
gFID $\downarrow$ & 2.244 & \textbf{2.242} & 0.1\%\\
$\fdr$ $\downarrow$ & 5.270 & \textbf{2.533} & 51.9\%\\
\midrule
\multicolumn{4}{@{}l}{\textit{80 generator epochs}}\\
gFID $\downarrow$ & 1.551 & \textbf{1.038} & 33.1\%\\
$\fdr$ $\downarrow$ & 3.375 & \textbf{1.856} & 45.0\%\\
\bottomrule
\end{tabular*}


==> HiRAE_Arxiv/analysis/tables/paired_reconstruction_intervals.tex <==
\begin{fullwidthtabular}{5}{lrrrr}
\toprule
Reference & $\Delta$PSNR & 95\% interval & $\Delta$LPIPS $\times10^3$ & 95\% interval\\
\midrule
RAEv2 & $+3.710$ & $[3.681, 3.742]$ & $-31.039$ & $[-31.327, -30.757]$\\
HiRAE-7 & $+1.309$ & $[1.292, 1.327]$ & $-6.389$ & $[-6.523, -6.257]$\\
\bottomrule
\end{fullwidthtabular}


==> HiRAE_Arxiv/analysis/tables/reconstruction_comparison.tex <==
\begin{fullwidthtabular}{5}{llrrr}
\toprule
Tokenizer & Configuration & rFID $\downarrow$ & PSNR (dB) $\uparrow$ & LPIPS $\downarrow$\\
\midrule
% \multicolumn{5}{l}{\textit{Published results}}\\
SD-VAE~\citep{yao2025vavae} & f8, 4 channels & 0.610 & 26.90 & 0.130\\
VA-VAE~\citep{yao2025vavae} & f16, 32 channels & 0.280 & 27.96 & 0.096\\
REPA-E~\citep{leng2025repae} & VA-VAE + E2E tuning & 0.280 & 26.25 & 0.110\\
RPiAE~\citep{gong2026rpiae} & Pivot + variational bridge & 0.500 & 21.30 & 0.216\\
FAE~\citep{gao2025fae} & 32-channel feature AE & 0.680 & \textendash & \textendash\\
RAE~\citep{zheng2025rae} & DINOv2-B, last layer & 0.570 & 18.80 & 0.256\\
DRoRAE~\citep{zhu2026drorae} & DINOv2-B, three-phase & 0.290 & 24.32 & 0.134\\
DecQ~\citep{wang2026decq} & DINOv2-B + 8 queries & 0.470 & 22.76 & \textendash\\
HAE~\citep{chang2026hae} & DINOv3-L, spherical latent & 0.780 & 25.20 & \textendash\\
\midrule
% \multicolumn{5}{l}{\textit{DINOv3-L: matched 5K PSNR/LPIPS; 50K rFID}}\\
RAEv2~\citep{singh2026raev2} & DINOv3-L, selected 7 layers & 0.299 & 22.667 & 0.074\\
\rowcolor{ourslight}\liftfull{} & DINOv3-L, all 24 layers & \textbf{0.209} & \textbf{26.377} & \textbf{0.043}\\
\bottomrule
\end{fullwidthtabular}


==> HiRAE_Arxiv/sections/00_teaser.tex <==
\noindent\begin{minipage}{\linewidth}
\centering
\includegraphics[width=0.80\linewidth]{figures/overview.pdf}
\captionsetup{hypcap=false}\captionof{figure}{\textbf{Learning full-depth fusion for higher reconstruction fidelity.} Top: HiRAE combines bounded residuals from three encoder-depth groups with the deepest-layer anchor. Left: matched input and reconstruction crops; HiRAE-24 reduces rFID by 30\% relative to RAEv2. Right: reconstruction and guided generation across systems under their respective reported settings.}
\label{fig:overview}
\end{minipage}
\par\vspace{4mm}


==> HiRAE_Arxiv/sections/01_opening.tex <==
\section{Introduction}
Pretrained vision encoders provide semantically organized representations for image generation, but their final outputs can omit details needed for faithful reconstruction~\citep{wang2026decq,singh2026raev2}. Representation Autoencoders (RAE)~\citep{zheng2025rae} pair these frozen encoders with learned decoders and train diffusion models in the resulting latent space. Many previous methods rely solely on the highly abstracted semantic features of the final encoder layer, whereas reconstruction depends more on the detailed features retained in intermediate layers~\citep{singh2026raev2,zhu2026drorae}. Learning to use this information offers a route to higher reconstruction fidelity while retaining the pretrained encoder as the basis for generation.
\par


==> HiRAE_Arxiv/sections/02_positioning.tex <==
% Using this hierarchical information requires deciding which layers to fuse and how to coordinate fusion learning with decoder training. 
Recent tokenizers exploit the visual hierarchy to recover details missing from final-layer representations, through fixed aggregation (RAEv2; \citealp{singh2026raev2}), learned full-depth fusion (DRoRAE; \citealp{zhu2026drorae}), or queries over intermediate features (DecQ; \citealp{wang2026decq}). IDEAL~\citep{chen2026ideal} combines selected shallow and deep features before quantization, while LV-RAE~\citep{liu2026lvrae} supplements semantic features with a separate encoder for low-level detail. DecQ shows that using shallower layers or increasing the number of detail queries can improve reconstruction while worsening generation. For learned fusion, this trade-off raises a further concern: reconstruction-driven training can favor shallow-layer detail without accounting for its effect on generation quality. Existing approaches reconcile reconstruction and generation through predefined layer aggregation, additional detail pathways, or staged adaptation of fusion and decoding. Our seven-layer experiments show that learned fusion improves reconstruction while supporting guided generation, but identifying a suitable layer subset requires repeated training and evaluation. We aim to learn a unified representation for reconstruction and generation through joint training of full-hierarchy fusion and the decoder. 
How can we learn full-hierarchy fusion that improves reconstruction while maintaining compatibility with generative modeling?
% How can we learn full-hierarchy fusion that improves reconstruction while controlling shallow-layer contributions and maintaining compatibility with generative modeling?

We introduce \lift{} (Hierarchical Representation Autoencoder), a hierarchical fusion framework that integrates representations across encoder depths into a shared latent space for reconstruction and generation. Its main configuration, \liftfull{}, learns spatially varying contributions from all 24 layers of a frozen DINOv3-L encoder, avoiding manual layer-subset selection. Building on DRoRAE's learned residual fusion~\citep{zhu2026drorae}, HiRAE organizes encoder layers into shallow, middle, and deep groups. Each group learns a residual correction to the deepest representation, with a distinct norm budget that increases with depth. These designs allow us to constrain how fusion modifies the deepest representation and jointly train the fusion module and decoder without a separate fusion-only adaptation phase. The fused representation preserves the original latent token count and channel dimension.
On ImageNet-256~\citep{deng2009imagenet}, \liftfull{} reduces rFID from 0.299 to 0.209, a 30\% reduction relative to RAEv2~\citep{singh2026raev2}. On the matched 5,000-image reconstruction subset, it increases PSNR from 22.667 to 26.377 dB and reduces LPIPS~\citep{zhang2018lpips} from 0.074 to 0.043. After 80 epochs of generator training, guided generation FID decreases from 1.060 to 1.038 (Figure~\ref{fig:overview}). Analysis shows that fusion adds spatial detail while largely preserving class neighborhoods. The learned tokenizer also exhibits lower decoding sensitivity to the tested latent perturbations.

Our contributions are:
\begin{itemize}
\item \textbf{Hierarchical representation autoencoding.} We introduce HiRAE, a hierarchical fusion framework with depth-dependent residual budgets. These budgets control intermediate-layer contributions to enrich the deepest representation with complementary visual detail.
\item \textbf{Higher reconstruction fidelity and improved text-to-image alignment.} \liftfull{} reduces reconstruction FID by 30\% relative to RAEv2 with competitive guided ImageNet generation. Under our shared text-to-image protocol, it improves GenEval, DPG-Bench, and GenAI-Bench scores before and after supervised fine-tuning, with a 2.84-point GenEval gain after fine-tuning.
\item \textbf{HiRAE's latent structure and decoding sensitivity.} Our analysis shows that hierarchical fusion enriches spatial detail while largely preserving class neighborhoods. The learned tokenizer also exhibits lower decoding sensitivity to the tested latent perturbations.
\end{itemize}

\section{Related work}
\paragraph{Visual representations for image generation.}
Latent diffusion models such as LDM and DiT generate images in the compressed spaces of reconstruction-trained autoencoders~\citep{rombach2022ldm,peebles2023dit}.
Representation alignment connects these generative models with pretrained visual encoders at different stages: REPA supervises diffusion features, whereas VA-VAE regularizes the tokenizer latents themselves~\citep{yu2025repa,yao2025vavae}.
Extending this connection to joint optimization, REPA-E uses alignment to support end-to-end tuning of the VAE and diffusion model~\citep{leng2025repae}.
RAE takes a more direct route by pairing a frozen vision encoder with a learned decoder and training diffusion in the encoder's representation space~\citep{zheng2025rae}.
HiRAE extends RAE with a learnable fusion module over the full frozen encoder hierarchy and jointly trains this module with the decoder.

\paragraph{Hierarchical fusion and detail enrichment.}
RAEv2~\citep{singh2026raev2} extends representation autoencoding through fixed aggregation of selected encoder layers, incorporating intermediate-layer detail into the representation used for reconstruction and generation.
The aggregation itself introduces no learned fusion module, making layer selection a key design choice.
Related detail-enrichment designs include shallow-deep fusion before quantization in IDEAL and additional detail representations in DecQ and LV-RAE~\citep{chen2026ideal,wang2026decq,liu2026lvrae}.
For learnable multi-layer fusion, DRoRAE combines layer-wise experts with routing across all encoder layers and trains the fusion module before adapting the decoder~\citep{zhu2026drorae}.
Building on this learned full-depth fusion, HiRAE introduces depth-dependent residual budgets that support joint fusion and decoder training.

\paragraph{Latent structure and generative modeling.}
Adding reconstruction detail also changes the representation that the generator must model, so improvements in reconstruction alone do not establish better generation~\citep{yao2025vavae,wang2026decq}.
FAE and HAE adapt pretrained representations for generation through feature compression and hyperspherical modeling, respectively~\citep{gao2025fae,chang2026hae}.
Complementing these architectural approaches, \citet{zhong2026diffusability} systematically examine how latent properties relate to generation quality across tokenizer families.
Our analysis examines this relationship within hierarchical fusion: we measure changes in spatial detail and class neighborhoods, together with the decoding response to latent perturbations.


==> HiRAE_Arxiv/sections/02b_continuation.tex <==
\begin{wrapfigure}[22]{r}{0.50\textwidth}
\vspace{-2\intextsep}
\centering
\includegraphics[width=\linewidth]{figures/continuation_design.pdf}
\caption{\textbf{Layer use and tokenizer training} in RAEv2, DRoRAE, and HiRAE-24.}
\label{fig:transition}
\end{wrapfigure}

% ROLE: overview | Connect learned full-hierarchy use and joint training to the fusion design.
\liftfull{} learns to use all encoder layers while jointly training the fusion module and decoder (Figure~\ref{fig:transition}). A separate learned transformation (expert) processes each layer's output, and a router learns the expert contributions at each spatial location. To prevent the latent space from drifting toward a reconstruction-dominated distribution during joint training, HiRAE combines these outputs into shallow, middle, and deep residual groups around the deepest-layer anchor. Group-wise norm caps assign tighter correction budgets to shallower groups, with residual dropout providing additional regularization. The encoder stays frozen, and the fused latent preserves its token count and channel dimension (Figure~\ref{fig:framework}).


==> HiRAE_Arxiv/sections/03_method.tex <==
\Needspace{0.46\textheight}
\section{HiRAE: controlled hierarchical composition}
\label{sec:method}
\input{sections/02b_continuation}



\subsection{Layer-wise experts}
\label{sec:layer_experts}
% ROLE: inherited definition | Retain the expert interface needed by routing and composition.
A separate token-wise MLP expert~\citep{zhu2026drorae} transforms each frozen encoder feature $H_\ell\in\mathbb{R}^{N\times C}$ before fusion:
\begin{equation}
 U_\ell=\mathcal{E}_\ell(H_\ell),
 \qquad \ell=0,\ldots,L-1.
 \label{eq:expert}
\end{equation}
We use all $L=24$ DINOv3-L~\citep{simeoni2025dinov3} layers with $N=256$ tokens and $C=1024$ channels; expert implementation details are given in Appendix~\ref{app:fusion_modules}.

\subsection{Routing}
% ROLE: component definition | Specify how spatial layer weights are computed.
A shared linear projection of the deepest feature $H_{L-1}$ produces routing scores at each spatial token $n$. We apply $\ell_2$ normalization to these scores, retaining their signs:
\begin{equation}
 a_n=\operatorname{Linear}_{R}(H_{L-1,n})\in\mathbb{R}^{L},
 \qquad w_n=\frac{a_n}{\norm{a_n}_2}.
 \label{eq:router}
\end{equation}
Stacking $w_n$ gives $W\in\mathbb{R}^{N\times L}$, whose column $w_\ell=W_{:,\ell}$ weights layer $\ell$ at each spatial location. Normalization details are given in Appendix~\ref{app:fusion_modules}.

\begin{figure}[tb]
\centering
\includegraphics[width=0.9\linewidth]{figures/raw24_framework_v1.pdf}
\caption{\textbf{HiRAE-24 architecture and training.} (a) Layer-wise experts and signed routing combine all 24 encoder layers under depth-dependent residual controls. (b) Tokenizer training jointly updates fusion and decoder while freezing the encoder. (c) Generator training freezes the tokenizer.}
\label{fig:framework}
\end{figure}


==> HiRAE_Arxiv/sections/04_training_setup.tex <==
\subsection{Residual regularization}
\label{sec:residual_controls}
% ROLE: motivation and design | Keep the learned full-depth correction around a deep anchor.
Routing controls the combination weights but does not directly bound the resulting feature correction. We retain $H_{L-1}$ as the anchor, but replace DRoRAE's global interpolation with \emph{residual regularization} applied separately to each depth group: groupwise norm caps and residual dropout. For the 24-layer encoder, we use three contiguous depth groups: $G_s=\{0,\ldots,7\}$, $G_m=\{8,\ldots,15\}$, and $G_d=\{16,\ldots,23\}$.

Each group forms an unregularized residual $R_g=\sum_{\ell\in G_g}w_\ell\odot U_\ell$, where $\odot$ broadcasts each spatial weight across channels. The residual-control module $\mathcal{C}_g$ converts $R_g$ into a controlled correction $\Delta_g$. We add these corrections to the deepest feature $H_{23}$ and apply layer normalization (LN) to obtain the fused latent $Z$:
\begin{equation}
 Z=\LN\!\left[H_{23}+\sum_{g\in\{s,m,d\}}\Delta_g\right],
 \qquad \Delta_g=\mathcal{C}_g(R_g;H_{23}),
 \label{eq:residual}
\end{equation}


Here, $\LN$ normalizes the $C$ channels of each spatial token independently. The module $\mathcal{C}_g$ first applies \emph{residual dropout} with probabilities $(p_s,p_m,p_d)=(0.50,0.25,0.10)$ during tokenizer training. It then scales down a group residual only when its norm exceeds its assigned budget. These \emph{groupwise norm caps} enforce
\begin{equation}
 \norm{\Delta_g}_F\leq c_g\norm{H_{23}}_F,
 \qquad (c_s,c_m,c_d)=(0.025,0.075,0.150).
 \label{eq:group_caps}
\end{equation}
Here, $\norm{\cdot}_F$ denotes the Frobenius norm, computed separately for each image over all spatial tokens and channels. The caps therefore bound the summed contribution of each depth group after routing. Shallower groups receive tighter norm budgets and stronger dropout, while middle and deep groups allow progressively larger corrections.

% ROLE: interpretation | Explain the depth-dependent budget without claiming generation guarantees.
Together, the three group budgets bound the total correction before final normalization. By the triangle inequality,
\begin{equation}
 \norm{\Delta_s+\Delta_m+\Delta_d}_F
 \leq \norm{\Delta_s}_F+\norm{\Delta_m}_F+\norm{\Delta_d}_F
 \leq 0.250\,\norm{H_{23}}_F.
 \label{eq:total_residual_bound}
\end{equation}
% Appendix~\ref{app:fusion_modules} provides implementation details.

\subsection{Training the tokenizer and generator}
\label{sec:training}
% ROLE: training | Explain what is optimized and when the tokenizer is frozen.
HiRAE jointly trains fusion and decoding within the tokenizer stage, then trains the generator on the frozen tokenizer's latents. In Stage 1, reconstruction losses update both the fusion module and decoder while the pretrained backbone stays frozen. DRoRAE~\citep{zhu2026drorae} instead trains fusion against a frozen decoder before decoder adaptation; HiRAE removes this separate fusion-only adaptation phase (Figure~\ref{fig:transition}). We use pixel reconstruction, perceptual, and adversarial losses, with decoder-input noise. In schematic form,
\begin{equation}
 \mathcal L_{\rm tok}=\mathcal L_{1}(x,\widehat x)
 +\lambda_{\rm perc}\mathcal L_{\rm perc}(x,\widehat x)
 +\lambda_{\rm adv}(e)\mathcal L_{\rm adv}(\widehat x).
\end{equation}
Here, $e$ denotes the training epoch. In Stage 2, we freeze the tokenizer and train a DiT generator on its latent representations, following RAEv2's prediction and internal-guidance framework. Appendix~\ref{app:implementation} provides the loss weighting and training configuration.

\section{Reconstruction and generation}
\label{sec:experiments}
% ROLE: dataset | Establish the dataset, resolution, and evaluation tasks.
\paragraph{Datasets.}
For reconstruction and class-conditional generation, we train and evaluate HiRAE on ImageNet-1K~\citep{deng2009imagenet}. For image reconstruction, we train the tokenizer on the training split at $256\times256$ resolution and evaluate on the validation split. Following the ADM evaluation protocol~\citep{dhariwal2021diffusion}, we generate 50,000 images per configuration for FID computation. For text-to-image (T2I) generation, we follow RAEv2~\citep{singh2026raev2} and pretrain on JourneyDB~\citep{sun2023journeydb} together with the long-caption and short-caption subsets of BLIP3o~\citep{chen2025blip3o}, using $256\times256$ images. We then apply supervised fine-tuning (SFT) on BLIP3o-60k.

% ROLE: metrics | Define the reported measures and their evaluation protocol.
\paragraph{Evaluation metrics.}
For ImageNet, we measure reconstruction quality with reconstruction FID (rFID), and generation quality with generation FID (gFID) and Inception Score (IS). On a matched reconstruction subset, we additionally measure peak signal-to-noise ratio (PSNR) and Learned Perceptual Image Patch Similarity (LPIPS; \citealp{zhang2018lpips}). We also report $\fdr$, which aggregates normalized Fr{\'e}chet distances across six representation spaces. Our evaluations use their arithmetic mean. For T2I, we evaluate text--image alignment with GenEval~\citep{ghosh2023geneval} and Dense Prompt Graph Benchmark (DPG-Bench; \citealp{hu2024ella}). We additionally report GenAI-Bench~\citep{li2024genaibench}, which evaluates compositional text--image alignment.

% ROLE: implementation | Specify model configurations, sampling, and reference-result conventions.
\paragraph{Implementation details.}
Our main comparisons evaluate \liftfull{}, which fuses all 24 layers of a frozen DINOv3-L encoder into a $16\times16\times1024$ latent. For ImageNet, we evaluate exponential moving average (EMA) generators with and without internal guidance, retaining class conditioning in both settings. Appendix~\ref{app:implementation} provides the ImageNet training and sampling configuration.
For T2I, we follow RAEv2. Pretraining uses 100K optimizer updates; SFT continues from the corresponding pretrained weights. Appendix~\ref{app:text_to_image} details training schedules and scoring protocols.

% Place the reconstruction examples with the reconstruction results.
\begin{figure}[!t]
\centering
% Compose the selected cases while preserving the complete source PDF.
\includegraphics[width=\linewidth]{figures/reconstruction_main.pdf}
\caption{\textbf{Matched reconstruction details.} Each selected triplet shows the input, official RAEv2, and HiRAE-24. Red boxes mark corresponding regions, enlarged below.}
\label{fig:reconstruction}
\end{figure}


==> HiRAE_Arxiv/sections/05_reconstruction.tex <==
\subsection{Reconstruction quality}
\label{sec:reconstruction}
\begin{table}[tb]
\centering
\caption{\textbf{ImageNet-256 reconstruction.} The upper block follows each source's evaluation protocol; dashes denote unreported values. The lower block combines 50K rFID with PSNR/LPIPS on our matched 5K subset (100 classes; AlexNet LPIPS). Bold marks the best result within the lower block.}
\label{tab:reconstruction}
\small
\input{analysis/tables/reconstruction_comparison}
\par\smallskip
% {\footnotesize $^{\dagger}$PSNR/LPIPS follow the SD-VAE and RAE-B evaluations in \citet[Table 3]{gong2026rpiae}.}
\end{table}

% ROLE: result and implication | Establish reconstruction headroom within a frozen hierarchy and fixed latent dimensions.
\textbf{HiRAE improves reconstruction fidelity within the original latent dimensions.} With the same frozen DINOv3-L encoder and $16\times16\times1024$ latent shape, \liftfull{} reduces rFID from the RAEv2 result of 0.299 to 0.209, a reduction of approximately 30\% (Table~\ref{tab:reconstruction}). On the matched 5,000-image subset, PSNR increases from 22.667 to 26.377 dB and LPIPS decreases from 0.074 to 0.043. The improvement therefore covers both pixel accuracy and perceptual similarity. Learned full-hierarchy fusion and joint decoder training recover finer image detail without increasing the generator's latent token count or channel dimension.
% ROLE: visual interpretation | Connect visible improvements in local appearance to the motivation for hierarchical fusion.
As shown in Figure~\ref{fig:reconstruction}, \liftfull{} more faithfully preserves text strokes and local colors. RAEv2 retains the overall image content but exhibits distortions in fine structures and local color shifts. These comparisons complement the rFID improvement, showing that controlled hierarchical fusion can recover image-specific details while maintaining the scene structure.
% ROLE: coverage | Connect selected examples to a systematic content-stratified analysis.
The improvement also extends across all four quartiles of original-image texture strength. More textured images show larger LPIPS reductions and a larger effect from removing the shallow residual group (Appendix~\ref{app:texture_strata}), complementing the visual examples.


==> HiRAE_Arxiv/sections/06_guided.tex <==
% Place the guided comparison with the generation results.

\Needspace{9\baselineskip}
\subsection{Image generation}
\label{sec:generation}
\input{sections/06_guided_table}
\input{sections/08_unguided}
% ROLE: generation results and design implications | Connect cross-system generation performance to token layout and representation-adaptation choices, then briefly report unguided results.
\textbf{Higher reconstruction fidelity coexists with competitive guided generation.}
As shown in Table~\ref{tab:guided}, \liftfull{} achieves a guided gFID of 1.038 after 80 epochs of generator training, compared with 1.060 for RAEv2 at the same training duration. IS also increases from 255.300 to 257.823. The reconstruction gain therefore coexists with competitive guided generation in the same representation learned from the full encoder hierarchy. DecQ~\citep{wang2026decq} appends eight detail-query tokens. It generates these alongside the original patch tokens, whereas \liftfull{} integrates hierarchical information into the existing patch-token layout. Their comparable gFID shows that detail enrichment can support competitive generation within the original latent token count and channel dimension. REPA-E~\citep{leng2025repae} obtains its tokenizer through end-to-end VAE--diffusion tuning; HiRAE learns fusion and decoding over a frozen encoder, then freezes the tokenizer for generator training. Figure~\ref{fig:guided_samples} shows selected outputs spanning animals, objects, and scenes, combining coherent object structure with fine local detail. Without guidance, Table~\ref{tab:unguided} shows that \liftfull{} achieves a gFID of 2.129, improving on RAEv2 K=23's 3.010 while remaining above RAEv2's 1.650.

\begin{figure}[tb]
\centering
% Display the upper half while preserving the complete source PDF.
\includegraphics[trim=0 182.4bp 0 0,clip,width=\linewidth]{figures/guided_samples.pdf}
\caption{\textbf{Guided samples from HiRAE-24.} Twenty-four selected class-conditioned images form eight visual groups, each with one larger example and two related samples.}
\label{fig:guided_samples}
\end{figure}


==> HiRAE_Arxiv/sections/06_guided_table.tex <==
\begin{table}[!t]
\centering
\caption{\textbf{Guided ImageNet-256 generation.} Epochs count generator training. CFG-int.: interval CFG; AG: AutoGuidance; IG: internal guidance.}
\label{tab:guided}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrlrrr}
\toprule
System & Epochs & Guide & gFID $\downarrow$ & IS $\uparrow$ & $\fdr$ $\downarrow$\\
\midrule
DiT-XL/2~\citep{peebles2023dit} & 1400 & CFG & 2.270 & 278.200 & ---\\
SiT-XL/2~\citep{ma2024sit} & 1400 & CFG & 2.060 & 270.300 & ---\\
REPA~\citep{yu2025repa} & 800 & CFG-int. & 1.420 & 305.700 & ---\\
VA-VAE~\citep{yao2025vavae} & 800 & CFG & 1.350 & 295.300 & ---\\
REPA-E~\citep{leng2025repae} & 800 & CFG & 1.120 & 302.900 & ---\\
RPiAE~\citep{gong2026rpiae} & 80 & AG & 1.510 & 225.900 & ---\\
FAE~\citep{gao2025fae} & 800 & CFG & 1.290 & 268.000 & ---\\
RAE~\citep{zheng2025rae} & 800 & AG & 1.130 & 262.600 & ---\\
RAE~\citep{zheng2025rae} & 80 & AG & 1.740 & 235.000 & ---\\
DRoRAE~\citep{zhu2026drorae} & 80 & AG & 1.650 & 230.600 & ---\\
LV-RAE~\citep{liu2026lvrae} & 800 & AG & 1.820 & 249.700 & ---\\
DecQ~\citep{wang2026decq} & 800 & AG & 1.050 & 259.600 & ---\\
HAE~\citep{chang2026hae} & 550 & CFG & 1.900 & 252.700 & ---\\
\midrule
\multicolumn{6}{l}{\textit{DINOv3-L / RAEv2 framework; internal guidance}}\\
RAEv2~\citep{singh2026raev2} & 80 & IG & 1.060 & 255.300 & 2.170\\
% RAEv2 K=23~\citep{singh2026raev2} & 80 & IG & 1.250 & 256.800 & ---\\
\rowcolor{ourslight}\liftfull{} & 80 & IG & \textbf{1.038} & \textbf{257.823} & \textbf{1.856}\\
\bottomrule
\end{tabular}
\end{table}


==> HiRAE_Arxiv/sections/07_text_to_image.tex <==
\subsection{Text-to-image generation}
\label{sec:text_to_image}
% ROLE: transfer setup | Test learned fusion under text conditioning before and after SFT.
HiRAE-7 and HiRAE-24 achieve higher text--image alignment scores than RAEv2 both after pretraining and after supervised fine-tuning (SFT). Table~\ref{tab:text_to_image} compares FLUX-VAE~\citep{labs2024flux}, RAEv2~\citep{singh2026raev2}, HiRAE-7, and \liftfull{} as frozen image tokenizers after 100K generator pretraining steps and after SFT. At inference, all four evaluated configurations use classifier-free guidance (CFG) with scale 6 and internal guidance disabled. We report GenEval, DPG-Bench, and GenAI-Bench scores; Appendix~\ref{app:text_to_image} gives implementation details.
After pretraining, \liftfull{} improves GenEval by 4.52 points and DPG-Bench by 1.51 points over RAEv2. This advantage persists after SFT, with gains of 2.84, 1.45, and 0.97 points on GenEval, DPG-Bench, and GenAI-Bench, respectively. HiRAE-7 also exceeds RAEv2 on every available benchmark, while \liftfull{} improves further across both stages. These results extend the evidence for learned fusion from class-conditioned generation to text-conditioned generation and support the full-depth configuration without prior layer-subset selection. Figure~\ref{fig:geneval_selected} in Appendix~\ref{app:qualitative_t2i} compares the four methods on five selected GenEval prompts after SFT.


\begin{table}[t]
\centering
\caption{\textbf{Text-to-image generation before and after SFT.} DPG and GenAI denote DPG-Bench and GenAI-Bench. Bold denotes the best available score within each stage.}
\label{tab:text_to_image}
\small
\begin{fullwidthtabular}{7}{lcccccc}
\toprule
 & \multicolumn{3}{c}{Pretraining} & \multicolumn{3}{c}{Finetuning}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Model & GenEval $\uparrow$ & DPG $\uparrow$ & GenAI $\uparrow$ & GenEval $\uparrow$ & DPG $\uparrow$ & GenAI $\uparrow$\\
\midrule
FLUX-VAE~\citep{labs2024flux} & 49.73& 78.86& 63.65& 84.13& 83.48& 68.75\\
RAEv2~\citep{singh2026raev2} & 56.42 & 81.22 & 67.02 & 84.86 & 84.90 & 71.69\\
HiRAE-7 & 58.77 & 81.60 & 67.13 & 85.17 & 85.05 & 72.02\\
\rowcolor{ourslight}\liftfull{} & \textbf{60.94} & \textbf{82.73} & \textbf{68.08} & \textbf{87.70} & \textbf{86.35} & \textbf{72.66}\\
\bottomrule
\end{fullwidthtabular}
\end{table}


==> HiRAE_Arxiv/sections/08_unguided.tex <==
\begin{wraptable}[7]{R}{0.5\textwidth}
\vspace{-\intextsep}
\setlength{\abovecaptionskip}{0pt}
\centering
\caption{\textbf{Unguided ImageNet-256 generation.}}
\label{tab:unguided}
\small
\setlength{\tabcolsep}{3pt}
\begin{fullwidthtabular}{4}{lrrr}
\toprule
Tokenizer & gFID $\downarrow$ & IS $\uparrow$ & $\fdr$ $\downarrow$\\
\midrule
RAEv2 & 1.650 & 228.000 & 3.950\\
RAEv2 K=23 & 3.010 & 206.000 & ---\\
\midrule
\rowcolor{ourslight}\liftfull{} & 2.129 & 210.339 & 4.660\\
\bottomrule
\end{fullwidthtabular}
\end{wraptable}


==> HiRAE_Arxiv/sections/09_discussion.tex <==
\section{Ablation Studies and Analysis}
\label{sec:discussion}

\subsection{Ablation studies}
\label{sec:fusion_designs}

\begin{table}[t]
\centering
\caption{\textbf{Expert inputs and residual regularization.} Raw-layer experts: $\checkmark$, 24 layer experts; $\times$, seven depth-mode experts. Residual regularization combines norm caps and residual dropout.}
\label{tab:ablations}
\small
\begin{fullwidthtabular}{8}{lccrrrrr}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{\shortstack{Raw-layer\\experts}} & \multirow{2}{*}{\shortstack{Residual\\regularization}} & \multirow{2}{*}{rFID $\downarrow$} & \multicolumn{2}{c}{20 epochs} & \multicolumn{2}{c}{80 epochs}\\
\cmidrule(lr){5-6}\cmidrule(lr){7-8}
 & & & & gFID $\downarrow$ & $\fdr$ $\downarrow$ & gFID $\downarrow$ & $\fdr$ $\downarrow$\\
\midrule
\rowcolor{ourslight}\lift{} & $\checkmark$ & $\checkmark$ & 0.209 & \textbf{2.242} & \textbf{2.533} & \textbf{1.038} & \textbf{1.856}\\
\lift{} & $\times$ & $\checkmark$ & 0.230 & 2.410 & 2.650 & 1.067 & 1.929\\
\lift{} & $\times$ & $\times$ & \textbf{0.023} & 7.905 & 14.722 & \textendash & \textendash\\
\bottomrule
\end{fullwidthtabular}
\end{table}

\begin{wraptable}[13]{R}{0.5\textwidth}
\setlength{\abovecaptionskip}{0pt}
\centering
\caption{\textbf{Fusion methods in the RAEv2 framework.} DRoRAE-style fusion uses global interpolation to mix the deepest-layer representation and aggregated expert output at a fixed 80:20 ratio.}
\label{tab:full_depth_composition}
\small
\begin{fullwidthtabular}{4}{lrrr}
\toprule
Model & rFID $\downarrow$ & gFID $\downarrow$ & $\fdr$ $\downarrow$\\
\midrule
\multicolumn{4}{l}{\textit{Selected 7 layers}}\\
RAEv2 & 0.299 & 1.060 & 2.170\\
HiRAE-7 & 0.217 & \textbf{1.038} & 1.913\\
\midrule
\multicolumn{4}{l}{\textit{All 24 layers}}\\
\shortstack[l]{RAEv2 + DRoRAE} & \textbf{0.065} & 1.551 & 3.375\\
\rowcolor{ourslight}\liftfull{} & 0.209 & \textbf{1.038} & \textbf{1.856}\\
\bottomrule
\end{fullwidthtabular}
\end{wraptable}

\paragraph{Comparison of fusion methods.}
Applying DRoRAE-style layer experts and learned aggregation~\citep{zhu2026drorae} within RAEv2 improves both reconstruction and guided generation (Table~\ref{tab:full_depth_composition}). On the same seven selected layers, HiRAE-7 reduces rFID from 0.299 to 0.217 and guided gFID from 1.060 to 1.038. HiRAE-24 uses all 24 layers to remove the prerequisite of selecting a suitable subset, while HiRAE-7 remains a compact extension when a subset is available. For full-depth fusion, we compare HiRAE-24 with DRoRAE-style fusion adapted to RAEv2, using 24 experts in both configurations. The adapted DRoRAE-style fusion achieves lower rFID (0.065 versus 0.209), whereas HiRAE-24 achieves lower guided gFID (1.038 versus 1.551) and $\fdr$ (1.856 versus 3.375). These results show that reconstruction fidelity alone is insufficient for choosing a fusion method for guided generation. HiRAE-24 improves reconstruction over RAEv2 while achieving competitive guided generation performance, supporting its use for both reconstruction and generation.

\paragraph{Expert input and residual regularization ablation.}
Table~\ref{tab:ablations} compares three configurations trained for 16 tokenizer epochs, with generation evaluated on 50K guided samples from EMA generators at epochs 20 and 80. With residual regularization fixed, replacing 24 raw-layer experts with seven depth-mode experts increases rFID from 0.209 to 0.230 and guided gFID from 1.038 to 1.067 at epoch 80. The same ordering holds at epoch 20, supporting retention of the layer-wise expert design. The unregularized depth-mode configuration reaches rFID 0.023, but its guided gFID and $\fdr$ rise to 7.905 and 14.722 at epoch 20, compared with 2.410 and 2.650 for the regularized configuration. Together, these comparisons favor retaining layer-wise experts and residual regularization to combine reconstruction fidelity with guided generation quality.


\paragraph{Depth-group ablation.}
We compare two, three, and four depth groups. Three groups achieve the lowest guided gFID, with rFID close to that of two groups (Table~\ref{tab:group_count_results}). This balance supports our three-group design. In the main HiRAE-24 tokenizer, removing any depth-group residual increases reconstruction LPIPS on 5,000 matched images (Table~\ref{tab:main_interventions}), showing that all three groups contribute to reconstruction. For equal-norm removals, high-frequency removal causes more damage in the shallow group, while low-frequency removal causes more damage in the deep group. The middle group's difference is small, with a paired 95\% interval that includes zero. These results support complementary reconstruction information across depths.
We provide full results in Apps~\ref{app:group_count} and~\ref{app:group_interventions}.
% Appendices~\ref{app:group_count} and~\ref{app:group_interventions} provide the protocols and full results.


\begin{table}[tb]
\begin{minipage}[t]{0.48\textwidth}
\vspace{0pt}
\centering
\caption{\textbf{Depth-group count.} rFID: 5K images; guided gFID: 10K samples, IG=1.78.}
\label{tab:group_count_results}
\small
\begin{fullwidthtabular}{3}{rrr}
\toprule
Groups & rFID $\downarrow$ & Guided gFID $\downarrow$\\
\midrule
2 & \textbf{3.293} & 29.385\\
\rowcolor{ourslight}3 & 3.363 & \textbf{28.354}\\
4 & 3.457 & 31.321\\
\bottomrule
\end{fullwidthtabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\vspace{0pt}
\centering
\caption{\textbf{Depth-group interventions.}
LPIPS changes $\times10^3$.}
\label{tab:main_interventions}
\small
\begin{fullwidthtabular}{3}{lrr}
\toprule
Depth group & \shortstack{Group removal} & High $-$ low\\
\midrule
Shallow (0--7) & 5.650 & 0.215\\
Middle (8--15) & 54.111 & 0.068\\
Deep (16--23) & 147.750 & $-2.053$\\
\bottomrule
\end{fullwidthtabular}
\end{minipage}
\end{table}

% \FloatBarrier
\subsection{Latent-space analysis}
\label{sec:latent_analysis}
% ROLE: representation evidence | Separate cross-system class organization from within-model spatial enrichment.
\textbf{Fusion expands spatial variation while retaining class organization.} Figure~\ref{fig:latent_analysis}(a) visualizes RAEv2 and \liftfull{} on the same 500 images using PHATE~\citep{moon2019phate}, which provides a low-dimensional visualization of the representations. In the original feature space, the same-class fraction among ten nearest neighbors over 5,000 matched images is 74.454\% for RAEv2 and 79.536\% for \liftfull{}.
Within \liftfull{}, this fraction changes from 79.634\% for the deep anchor to 79.536\% after fusion, indicating largely preserved class neighborhoods. Across 100 fixed images, one per class, spatial effective rank increases from 130.360 for the deep anchor, $\LN(H_{23})$, to 154.893 for the fused representation, with an increase in every image (Figure~\ref{fig:latent_analysis}(b)). Meanwhile, mean spatial centered kernel alignment (CKA; \citealp{kornblith2019similarity}) remains 0.985. Thus, spatial variation spreads over more feature directions while the patch-relationship structure remains similar.
% Appendix~\ref{app:feature_geometry} specifies the estimators and normalization controls.

\begin{figure}[t]
\centering
\includegraphics[width=0.90\linewidth]{figures/latent_geometry_and_decoding.pdf}
% \caption{\textbf{Latent structure and decoding sensitivity.}
% (a) PHATE views colored by class; 10NN measures same-class neighbor agreement.
% (b) Anchor--fusion effective rank and CKA measure spatial variation dimensionality and structural similarity. Lines pair images; points and bars show means and 95\% bootstrap CIs.
% (c) Mean LPIPS between clean and perturbed decodings at 10\% relative latent perturbation norm; lower values indicate lower sensitivity.}
\caption{\textbf{Latent structure and decoding sensitivity.} (a) Independently fitted PHATE views of the same images; colors denote classes. Same-class 10NN uses the original feature space. (b) Within HiRAE-24, lines connect anchor--fusion effective ranks for 100 images; points and error bars show means and 95\% bootstrap CIs. (c) Mean output LPIPS under 10\% relative latent perturbations.}
\label{fig:latent_analysis}
\end{figure}

% ROLE: decoding evidence | Distinguish reconstruction detail from response to controlled latent deviations.
\textbf{Spatial enrichment coexists with lower decoding sensitivity.} Figure~\ref{fig:latent_analysis}(c) measures LPIPS between clean and perturbed decodings under Gaussian, low-frequency, and high-frequency latent perturbations. We measure each tokenizer's decoding response through its own inverse normalization and trained decoder. At a perturbation norm equal to 10\% of the standardized latent norm, \liftfull{} produces 21\%--22\% of RAEv2's output LPIPS change across the three direction types.
% ROLE: prediction evidence | Check the trained generator without treating forward-noising error as sample quality.
The trained generator also predicts \liftfull{} latents more accurately across intermediate noise levels. At seven matched coefficient log signal-to-noise ratio (log-SNR) levels, \liftfull{} has lower clean-latent mean squared error than RAEv2 at the five interior levels and slightly higher error at both endpoints. Appendix~\ref{app:mechanism} provides the full results and protocol. The diagnostics show lower latent prediction error at intermediate noise levels and lower decoding sensitivity to the perturbations.


==> HiRAE_Arxiv/sections/11_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
HiRAE learns high-fidelity visual tokenizers through joint fusion and decoder training, with depth-dependent residual bounds controlling each depth group's contribution. HiRAE-24 learns the contributions of all 24 encoder layers without manual layer-subset selection or a separate fusion-only adaptation phase. ImageNet-256 results show higher reconstruction fidelity than RAEv2 with competitive guided generation within the original latent dimensions. Matched-image analyses connect the added detail to complementary information across depth groups and largely preserved class neighborhoods. HiRAE-7 extends the framework to compact fusion over an established subset.
% % ROLE: conclusion | Close on reconstruction fidelity, learned full-hierarchy use, and joint tokenizer training.
% HiRAE learns high-fidelity visual tokenizers from the full encoder hierarchy through joint fusion and decoder training. HiRAE-24 learns the contributions of all 24 encoder layers without manual layer-subset selection or a separate fusion-only adaptation phase. During joint training, depth-dependent residual bounds control each depth group's contribution to the fused representation. ImageNet-256 results show higher reconstruction fidelity than RAEv2 with competitive guided generation within the original latent dimensions. 
% Matched-image analyses connect the added detail to complementary information across depth groups and largely preserved class neighborhoods. 
% HiRAE-7 extends the framework to compact fusion over an established subset.
% % ROLE: future work | Identify extensions across encoder families and training scales.
% Future work can examine learned fusion across encoder families and at larger training scales.


==> HiRAE_Arxiv/sections/abstract.tex <==
Pretrained visual representations support image generation, but may not fully preserve the fine-grained details needed for faithful reconstruction. Meanwhile, intermediate encoder layers contain complementary visual details, but learning to fuse them for reconstruction can produce a latent distribution that is difficult to model. Existing fusion methods require empirical tuning of layer selection or staged optimization of fusion and decoding, increasing configuration effort or training complexity. We introduce \lift{} (Hierarchical Representation Autoencoder), which learns a hierarchical fusion framework over the full encoder hierarchy to improve reconstruction fidelity while maintaining compatibility with generative modeling. HiRAE groups encoder layers by depth and learns residual corrections to the deepest representation. Group-wise norm caps bound these corrections relative to the deep anchor, with tighter budgets for shallower groups. Our \liftfull{} preserves the latent token count and channel dimension. On ImageNet-256, \liftfull{} reduces reconstruction FID from 0.299 to 0.209 relative to RAEv2 while maintaining competitive guided generation quality.
For text-to-image generation, \liftfull{} improves alignment over RAEv2 on GenEval, DPG-Bench, and GenAI-Bench both before and after supervised fine-tuning. Under the same generator-training and evaluation protocol, post-fine-tuning GenEval increases from 84.86 to 87.70.

